Generating Compact Geometric Track-Maps for Train Positioning Applications

In this paper, we present a method to generate compact geometric track-maps for train-borne localization applications. Therefore, we first give a brief overview on the purpose of track maps in train-positioning applications. It becomes apparent that there are hardly any adequate methods to generate suitable geometric track-maps. This is why we present a novel map generation procedure. It uses an optimization formulation to find the continuous sequence of track geometries that fits the available measurement data best. The optimization is initialized with the results from a localization filter developed in our previous work. The localization filter also provides the required information for shape identification and measurement association. The presented approach will be evaluated on simulated data as well as on real measurements.

==> tables/final_track_map.tex <==
% This table requires: \usepackage{siunitx}
\begin{threeparttable}
    \renewcommand{\arraystretch}{1.3}
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{|r||c|c|c|c|c|c|c|ccc|c|} \hline
        Track ID                               & $1$         & $2$         & $3$         & $4$         & $5$         & $6$         & $7$         & & \ldots & & $53$     \\ \hline 
        Shape\tnote{a}\hspace{0.5em}           & st          & ta          & ca          & ta          & st          & ta          & ca          & & \ldots & & st       \\ \hline
        Length $L$ in m                        & $0$         & $11$        & $27$        & $25$        & $218$       & $76$        & $136$       & & \ldots & & $296$    \\ \hline
        Radius\tnote{b}\hspace{0.5em} $r$ in m & ---         & $213$       & $213$       & $213$       & ---         & $376$       & $376$       & & \ldots & & ---      \\ \hline
        Latitude $\varphi_0$ in $^\circ$       & $50.548$    & ---         & ---         & ---         & ---         & ---         & ---         & & \ldots & & ---      \\ \hline
        Longitude $\lambda_0$ in $^\circ$      & $12.913$    & ---         & ---         & ---         & ---         & ---         & ---         & & \ldots & & ---      \\ \hline
        Heading $\Psi_0$ in $^\circ$           & $231.2$     & ---         & ---         & ---         & ---         & ---         & ---         & & \ldots & & ---      \\ \hline
    \end{tabular}
    %
    \scriptsize
    \begin{tablenotes}
        \item[a] st: straight, ta: transitional arc, ca: circular arc
        \item[b] the sign indicates the turning direction ($+$ right, $-$ left)
    \end{tablenotes} 
\end{threeparttable}

==> tables/optim_track_map.tex <==
% This table requires: \usepackage{siunitx}
\begin{threeparttable}
    \renewcommand{\arraystretch}{1.3}
    \setlength{\tabcolsep}{0.5pt}
    \begin{tabular}{|r||c|c|c|c|c|c|c|c|c|} \hline
        Track ID                               & $1$         & $2$         & $3$         & $4$         & $5$         & $6$         & $7$         & $8$         & $9$         \\ \hline %\hhline{|=||=|=|=|=|=|=|=|=|=|}
        Shape\tnote{a}\hspace{0.5em}           & st          & ta          & ca          & ta          & st          & ta          & ca          & ta          & st          \\ \hline
        Length $L$ in m                        & $1023$      & $260$       & $431$       & $209$       & $991$       & $216$       & $128$       & $175$       & $983$       \\ \hline
        Radius $r$ in m & $\infty$             & $-850$      & $-850$      & $-850$      & $\infty$    & $309$         & $309$     & $309$         & $\infty$    \\ \hline
        Start point $\xi_0$ in m               & $0$         & ---         & ---         & ---         & ---         & ---         & ---         & ---         & ---         \\ \hline
        Start point $\eta_0$ in m              & $-1$        & ---         & ---         & ---         & ---         & ---         & ---         & ---         & ---         \\ \hline
        Orientation $\varphi_0$ in $^\circ$    & $10.2$      & ---         & ---         & ---         & ---         & ---         & ---         & ---         & ---         \\ \hline
    \end{tabular}
    %
    \begin{tablenotes}
        \item[a] st: straight, ta: transitional arc, ca: circular arc
%         \item[b] the sign indicates the turning direction ($+$ right, $-$ left)
    \end{tablenotes} 
\end{threeparttable}

==> tables/reparam_optim_track_map.tex <==
% This table requires: \usepackage{siunitx}
\begin{threeparttable}
    \renewcommand{\arraystretch}{1.3}
    \setlength{\tabcolsep}{0.5pt}
    \begin{tabular}{|r||c|c|c|c|c|c|c|c|c|} \hline
        Track ID                               & $1$         & $2$         & $3$         & $4$         & $5$         & $6$         & $7$         & $8$         & $9$         \\ \hline %\hhline{|=||=|=|=|=|=|=|=|=|=|}
        Shape\tnote{a}\hspace{0.5em}           & st          & ta          & ca          & ta          & st          & ta          & ca          & ta          & st          \\ \hline
        Length $L$ in m                        & ---         & $260$       & $431$       & $209$       & ---         & $216$       & $128$       & $175$       & ---         \\ \hline
        Radius\tnote{b}\hspace{0.5em} $r$ in m & ---         & ---         & $-850$      & ---         & ---         & ---         & $309$       & ---         & ---         \\ \hline
        Start point $\xi_0$ in m               & $0$         & ---         & ---         & ---         & $1742$      & ---         & ---         & ---         & $2743$      \\ \hline
        Start point $\eta_0$ in m              & $-1$        & ---         & ---         & ---         & $640$       & ---         & ---         & ---         & $1664$      \\ \hline
        End point $\xi_e$ in m                 & $1007$      & ---         & ---         & ---         & $2310$      & ---         & ---         & ---         & $3722$      \\ \hline
        End point $\eta_e$ in m                & $180$       & ---         & ---         & ---         & $1452$      & ---         & ---         & ---         & $1579$      \\ \hline
    \end{tabular}
    %
    \begin{tablenotes}
        \item[a] st: straight,~~ta: transitional arc,~~ca: circular arc
        \item[b] the sign indicates the turning direction ($+$ right, $-$ left)
    \end{tablenotes} 
\end{threeparttable}

==> tables/track_map_quality.tex <==
\begin{tabular}{rcccc}
    \toprule
                       & $mean(|\epsilon|)$   & CDF$_{\text{0.95}}$ & CDF$_{\text{0.99}}$ & CDF$_{\text{1.00}}$ \\ \cmidrule(lr){1-5}
    $|\epsilon|$\,in m & $1.8$                & $5.7$               & $7.5$               & $8.7$               \\
    \bottomrule
\end{tabular}

